Enhanced Preheating after Multi-Field Inflation: On the Importance of being Special

We discuss preheating after multi-field inflation in the presence of several preheat matter fields that become light in the vicinity of (but not at) the inflatons' VEV, at distinct extra-species-points (ESP); this setup is motivated by inflationary models that include particle production during inflation, e.g.trapped inflation, grazing ESP encounters or modulated trapping, among others. While de-phasing of inflatons tends to suppress parametric resonance, we find two new effects leading to efficient preheating: particle production during the first in-fall (efficient if many preheat matter fields are present) and a subsequent (narrow) resonance phase (efficient if an ESP happens to be at one of several distinct distances from the inflatons' VEV). Particles produced during the first in-fall are comprised of many species with low occupation number, while the latter are made up of a few species with high occupation number. We provide analytic descriptions of both phases in the absence of back-reaction, which we test numerically. We further perform lattice simulations to investigate the effects of back-reaction. We find resonances to be robust and the most likely cause of inflaton decay in multi-field trapped inflation if ESP distributions are dense.

==> pnd_comparison.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7936.00,3400.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}-50}}%
      \put(946,947){\makebox(0,0)[r]{\strut{} 0}}%
      \put(946,1190){\makebox(0,0)[r]{\strut{} 50}}%
      \put(946,1433){\makebox(0,0)[r]{\strut{} 100}}%
      \put(946,1676){\makebox(0,0)[r]{\strut{} 150}}%
      \put(946,1920){\makebox(0,0)[r]{\strut{} 200}}%
      \put(946,2163){\makebox(0,0)[r]{\strut{} 250}}%
      \put(946,2406){\makebox(0,0)[r]{\strut{} 300}}%
      \put(946,2649){\makebox(0,0)[r]{\strut{} 350}}%
      \put(946,2892){\makebox(0,0)[r]{\strut{} 400}}%
      \put(946,3135){\makebox(0,0)[r]{\strut{} 450}}%
      \put(1078,484){\makebox(0,0){\strut{} 0}}%
      \put(1577,484){\makebox(0,0){\strut{} 0.2}}%
      \put(2075,484){\makebox(0,0){\strut{} 0.4}}%
      \put(2574,484){\makebox(0,0){\strut{} 0.6}}%
      \put(3072,484){\makebox(0,0){\strut{} 0.8}}%
      \put(3571,484){\makebox(0,0){\strut{} 1}}%
      \put(176,1919){\rotatebox{-270}{\makebox(0,0){\strut{}$n_k$}}}%
      \put(2324,154){\makebox(0,0){\strut{}$t$ [$N$]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(4782,704){\makebox(0,0)[r]{\strut{}-4}}%
      \put(4782,1008){\makebox(0,0)[r]{\strut{}-2}}%
      \put(4782,1312){\makebox(0,0)[r]{\strut{} 0}}%
      \put(4782,1616){\makebox(0,0)[r]{\strut{} 2}}%
      \put(4782,1920){\makebox(0,0)[r]{\strut{} 4}}%
      \put(4782,2223){\makebox(0,0)[r]{\strut{} 6}}%
      \put(4782,2527){\makebox(0,0)[r]{\strut{} 8}}%
      \put(4782,2831){\makebox(0,0)[r]{\strut{} 10}}%
      \put(4782,3135){\makebox(0,0)[r]{\strut{} 12}}%
      \put(4914,484){\makebox(0,0){\strut{} 0}}%
      \put(5439,484){\makebox(0,0){\strut{} 2}}%
      \put(5964,484){\makebox(0,0){\strut{} 4}}%
      \put(6489,484){\makebox(0,0){\strut{} 6}}%
      \put(7014,484){\makebox(0,0){\strut{} 8}}%
      \put(7539,484){\makebox(0,0){\strut{} 10}}%
      \put(4144,1919){\rotatebox{-270}{\makebox(0,0){\strut{}$\ln{(n_k)}$}}}%
      \put(6226,154){\makebox(0,0){\strut{}$t$ [$N$]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{pnd_comparison1}}%
    \gplfronttext
  \end{picture}%
\endgroup

